Query-guided End-to-End Person Search

Person search has recently gained attention as the novel task of finding a person, provided as a cropped sample, from a gallery of non-cropped images, whereby several other people are also visible. We believe that i. person detection and re-identification should be pursued in a joint optimization framework and that ii. the person search should leverage the query image extensively (e.g. emphasizing unique query patterns). However, so far, no prior art realizes this. We introduce a novel query-guided end-to-end person search network (QEEPS) to address both aspects. We leverage a most recent joint detector and re-identification work, OIM [37]. We extend this with i. a query-guided Siamese squeeze-and-excitation network (QSSE-Net) that uses global context from both the query and gallery images, ii. a query-guided region proposal network (QRPN) to produce query-relevant proposals, and iii. a query-guided similarity subnetwork (QSimNet), to learn a query-guided reidentification score. QEEPS is the first end-to-end query-guided detection and re-id network. On both the most recent CUHK-SYSU [37] and PRW [46] datasets, we outperform the previous state-of-the-art by a large margin.

==> acknowledgements.tex <==
\section{Acknowledgements}



==> latex/fig/QRPN2.tex <==
\begin{figure}[t] 
\begin{center}
	\includegraphics[trim=0cm 0cm 16cm 0cm, clip=true, width=0.8\linewidth]{latex/fig/QRPN2_fig.pdf}
	\caption{Query-guided RPN. $r = 16$}\label{fig:qrpn}
	\vspace{-10pt}
\end{center}
\end{figure}


==> latex/fig/results_qsse.tex <==
\tabcolsep 1.0pt
\renewcommand{\arraystretch}{1}

\newlength{\cuhkfigheightfail}
\setlength{\cuhkfigheightfail}{2cm}

\begin{figure*}[h]
\begin{center}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}{ccc|ccc}

\includegraphics[trim=0cm 0cm 2cm 2cm, clip=true, height=\cuhkfigheight]{latex/fig/results/1294_s7714_gt_3.jpg}&
\includegraphics[trim=0cm 0cm 0cm 5cm, clip=true, height=\cuhkfigheight]{latex/fig/results/1294_s7714_ours_without_qsse_top0.jpg}&
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true, height=\cuhkfigheight]{latex/fig/results/1294_s7714_ours_top0.jpg}&

\includegraphics[trim=0cm 13cm 0cm 1cm, clip=true, height=\cuhkfigheight]{latex/fig/results/2890_s10359_gt_1.jpg}&
\includegraphics[trim=0cm 0cm 0cm 5cm, clip=true, height=\cuhkfigheight]{latex/fig/results/2890_s10359_ours_without_qsse_top0.jpg}&
\includegraphics[trim=0cm 13cm 0cm 1.2cm, clip=true, height=\cuhkfigheight]{latex/fig/results/2890_s10359_ours_top0.jpg}\\

Query & QEEPS \textit{w/o} QSSE & QEEPS & Query & QEEPS \textit{w/o} QSSE & QEEPS    \\ 

\end{tabular}

\caption{Here }

\vspace{-0.5cm}
\label{fig:qsse_results_v1}
\end{center}
\end{figure*}


%\setlength{\cuhkfigheight}{2cm}

==> latex/tables/res_prw.tex <==
\begin{table}
\begin{center}
\begin{tabular}{|l|c|c|c|}
\hline
Method & mAP(\%) & top-1 (\%) \\
\hline\hline
OIM \cite{xiao2017joint}  & 21.3 & 49.9 \\
IAN \cite{Xiao2017IANTI} & 23.0 & 61.9  \\
NPSM \cite{Liu2017NPSM} & 24.2 & 53.1 \\
Mask-G \cite{Chen_2018_ECCV} & 32.6 & 72.1 \\
\hline
Ours (\textit{resnet50+}) & 0 & 0 \\
\hline
\end{tabular}
\end{center}
\caption{Comparison to the state-of-the-art on PRW Dataset}
\end{table}


==> latex/tables/res_prwmini_more_data.tex <==
\begin{table}
\begin{center}
\begin{tabular}{lcc}
\hline
Method & mAP(\%) & top-1 (\%) \\
\hline
\hline
% OIM \cite{xiao2017joint}  & 21.3 & 49.9 \\
% IAN \cite{Xiao2017IANTI} & 23.0 & 61.9  \\
% NPSM \cite{Liu2017NPSM} & 24.2 & 53.1 \\
% Mask-G \cite{Chen_2018_ECCV} & 32.6 & 72.1 \\
% OIM\ddag\ (Baseline) &  36.9 & 75.7\\
% QEEPS (ours)& _ & _ \\
% \hdashline[3pt/5pt]
Mask-G \cite{Chen_2018_ECCV} & 33.1 & 70.0 \\
OIM\ddag\ (Baseline) & 38.3 & 70.0 \\
+ \textit{QSimNet} & 38.4 & 66.7\\
%+ \textit{QRPN} + \textit{QSimNet} & 37.3 & 73.3\\

QEEPS (ours)& \bf{40.7} & \bf{73.3} \\
\hline
\end{tabular}
\end{center}
\caption{Comparison with the state-of-the-art on the proposed subset PRW-mini using more data for training.}
\label{tab:sota_prw_more_data}
\vspace{-0.5cm}
\end{table}







